Defect measures of eigenfunctions with maximal $ L^\infty $ growth

We study the relationship between $L^\infty$ growth of eigenfunctions and their $L^2$ concentration as measured by defect measures. In particular, we characterize the defect measures of any sequence of eigenfunctions with maximal $L^\infty$ growth, showing that they must be neither more concentrated nor more diffuse than the zonal harmonics. As a consequence, we obtain new proofs of results on the geometry manifolds with maximal eigenfunction growth obtained by Sogge--Zelditch, and Sogge--Toth--Zelditch.

==> paper_commands.tex <==
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{amsthm}
\usepackage{amsxtra}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{comment}
\usepackage{url}
\pagestyle{headings}
\usepackage{color}
%\usepackage{dsfont}
\usepackage[notref,notcite,color]{showkeys}

\usepackage[colorlinks=true, citecolor=red]{hyperref}
\usepackage{amsfonts}
\usepackage{textcomp}
\usepackage{perpage,enumerate}

\usepackage{caption}
\usepackage{subcaption}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\usepackage{lmodern}

\usepackage{sidecap}

\setlength{\textheight}{8.00in} \setlength{\oddsidemargin}{0.0in}
\setlength{\evensidemargin}{0.0in} \setlength{\textwidth}{6.4in}
\setlength{\topmargin}{0.18in} \setlength{\headheight}{0.18in}
\setlength{\marginparwidth}{1.0in}
\setlength{\abovedisplayskip}{0.2in}

\setlength{\belowdisplayskip}{0.2in}

\setlength{\parskip}{0.05in}
%\textwidth = 15cm              




\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator*{\oph}{Op_h}
\DeclareMathOperator*{\diam}{diam}
\DeclareMathOperator*{\op}{Op}
\DeclareMathOperator*{\supp}{supp}
\DeclareMathOperator*{\WF}{WF}
\DeclareMathOperator*{\WFh}{WF_h}
\DeclareMathOperator*{\loc}{loc}
\DeclareMathOperator*{\comp}{comp}
\DeclareMathOperator*{\Ell}{ell}
\DeclareMathOperator*{\MS}{MS_h}
\DeclareMathOperator*{\graph}{graph}
\DeclareMathOperator*{\sgn}{sgn}
\DeclareMathOperator*{\Id}{Id}
%\DeclareMathOperator*{\det}{det}
\DeclareMathOperator*{\tr}{tr}
\DeclareMathOperator*{\Arg}{Arg}


\usepackage{chngcntr}

\graphicspath{{Figures/}}

\newcommand{\Lsection}[1]{\section[#1]{{\Large{#1}}}}


\def\smallsection#1{\smallskip\noindent\textbf{#1}.}
\def\bigsection#1{\smallskip\noindent{\textbf{#1}.}\smallskip}

\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\numberwithin{prop}{section}
\newtheorem{corol}{Corollary}
\numberwithin{corol}{section}


\newtheorem{lemma}{Lemma}
\numberwithin{lemma}{section}
\newtheorem{conjecture}{Conjecture}
\numberwithin{conjecture}{section}

\newenvironment{remarks}[1][]{\begin{remark}\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]\end{trivlist}\begin{itemize}}{\end{itemize}\end{remark}}

{\theoremstyle{definition}
\newtheorem{defin}{Definition}
\numberwithin{defin}{section}
}
\numberwithin{figure}{section}


%\counterwithout{equation}{section}
%\counterwithout{subsection}{section}
%\counterwithout{figure}{section}

\renewcommand{\Re}{\mathop{\rm Re}\nolimits}
\renewcommand{\Im}{\mathop{\rm Im}\nolimits}

%new commands

\newcommand{\quotient}[2]{{\left.\raisebox{.2em}{$#1$}\middle/\raisebox{-.2em}{$#2$}\right.}}

\newcommand{\CI}{C^\infty}
\newcommand{\CIc}{C^\infty_{\rm{c}}}
\newcommand{\RR}{\mathbb R}
\newcommand{\Spec}{\operatorname{Spec}}
\newcommand{\bl}{\begin{flushleft}}
\newcommand{\el}{\end{flushleft}}
\newcommand{\br}{\begin{flushright}}
\newcommand{\ert}{\end{flushright}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\nq}{\vspace{1cm}}%new question
\newcommand{\nsq}{\vspace{5mm}}%new subquestion
\newcommand{\union}{\bigcup}
\newcommand{\isect}{\bigcap}
\newcommand{\mcal}[1]{\mathcal{#1}}
\newcommand{\unionLim}[3]{\union _{#1=#2}^{#3}}
\newcommand{\isectLim}[3]{\isect _{#1=#2}^{#3}}
\newcommand{\recip}[1]{\frac{1}{#1}}
\newcommand{\imply}{\Rightarrow}
\newcommand{\iaof}{\Leftrightarrow}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\numList}{\begin{enumerate}}
\newcommand{\enumList}{\end{enumerate}}
\newcommand{\sumLim}[3]{\sum_{#1=#2}^{#3}}
\newcommand{\liml}[2]{\lim_{#1 \to #2}}
\newcommand{\st}{\backepsilon}
\newcommand{\imat}{\left( \begin{array}{cc}0&-i\\i&0\\ \end{array}\right)}
\newcommand{\composed}{\text{\textopenbullet}}
\newcommand{\cross}{\times}
\newcommand{\e}{\epsilon}
\newcommand{\pf}{\textbf{Proof:}}
\newcommand{\lem}{\textbf{Lemma:}}
\newcommand{\cor}{\textbf{Corollary:}}
\newcommand{\intL}[2]{\int_{#1}^{#2}}
\newcommand{\re}{\mathbb{R}}
\newcommand{\poin}{Poincar\'{e} }
\newcommand{\nn}{\nonumber\\}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\Dloc}{\mathcal{D}_{\loc}}
\newcommand{\negint}{{\int\negthickspace\negthickspace\negthickspace\negthinspace -}}
\newcommand{\cald}{Calder\'{o}n }
\newcommand{\fint}{-\!\!\!\!\!\!\int}
\newcommand{\PsiHom}{\Psi_{\textup{hom}}}


\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\pO}{\partial\Omega}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newcommand{\Deltap}{\Delta_{\partial\Omega,\delta'}}
\newcommand{\Deltad}[1]{\Delta_{#1,\delta}}
\newcommand{\sech}{\operatorname{sech}}
\newcommand{\asec}{\operatorname{arcsec}}
\newcommand{\Fh}{\mc{F}_h}

\newcommand{\dDl}{\partial_{\nu}\mc{D}\ell}
\newcommand{\Dl}{N}
\newcommand{\Sl}{\mc{S}\ell}
\newcommand{\D}{\mc{D}\ell}
\renewcommand{\S}{\mc{S}\ell}
\newcommand{\Cc}{C_c^\infty}
\renewcommand{\O}[1]{\mathpzc{O}_{#1}}
\renewcommand{\o}[1]{\mathpzc{o}_{#1}}
\newcommand{\opht}[1]{\operatorname{Op_{h,#1}}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\No}{N_2}
\newcommand{\Ph}[2]{\Psi^{#1}_{#2}}
\newcommand{\Do}{D_{\Omega}}
\newcommand{\m}{$$}
